Found by Search, Broken by a Shortcut: Transfer and Tampering of Searched Intrinsic Rewards

Can a search over innate drives find intrinsic rewards that help a reinforcement-learning agent learn, transfer to a task it never saw, and resist an exploit that was absent during the search? Each candidate reward combines four generic events (a new view, a pickup, a drop and a toggle), each with a weight, a relief and a refill rate. We ran three pre-registered stages; the search protocol was locked in a public, timestamped commit before any search result existed. CMA-ES and an equal-budget random search used 1,560 PPO training runs, and the final evaluation and tamper test used 340. On the held-out task, KeyCorridorS3R2, the CMA-ES-selected reward (E) beat task-only PPO, episodic novelty and the random-search-selected reward (R) in all 3 registered comparisons, all of them meaningful by the registered size rule. Among these generic rewards E transferred best; the earlier paper's satiation reward, which on this task is given hand-wired key and locked-door events, did better (20 of 20 seeds solved against 4 of 20; descriptive). On UnlockPickup, where that reward uses generic events, E's mean area exceeded it by 0.276 (descriptive). On the training tasks there was no registered difference between E and R: both E-over-R tests missed. A free reset action, absent during the search, collapsed E's learning on DoorKey-8x8 (mean area 0.829 without it, 0.136 with it; registered) to below task-only PPO (descriptive). The searched drives helped on every task tested, but a reward given task-specific events did better on the held-out task, and selection gave E no protection against an exploit absent from the search.

==> numbers.tex <==
% Generated by scripts/make_numbers.py from data/raw. Do not edit by hand.
\makeatletter
\@namedef{val@s2.runs}{1,560}\@namedef{line@s2.runs}{2}
\@namedef{val@s2.search}{1,440}\@namedef{line@s2.search}{3}
\@namedef{val@s2.searchcma}{720}\@namedef{line@s2.searchcma}{4}
\@namedef{val@s2.searchrand}{720}\@namedef{line@s2.searchrand}{5}
\@namedef{val@s2.reeval}{120}\@namedef{line@s2.reeval}{6}
\@namedef{val@s2.reevalper}{60}\@namedef{line@s2.reevalper}{7}
\@namedef{val@s2.cands}{120}\@namedef{line@s2.cands}{8}
\@namedef{val@s2.candtotal}{240}\@namedef{line@s2.candtotal}{9}
\@namedef{val@s2.gens}{12}\@namedef{line@s2.gens}{10}
\@namedef{val@s2.finalists}{3}\@namedef{line@s2.finalists}{11}
\@namedef{val@s2.conc}{32}\@namedef{line@s2.conc}{12}
\@namedef{val@s2.pop}{10}\@namedef{line@s2.pop}{13}
\@namedef{val@s2.mean0}{0.5}\@namedef{line@s2.mean0}{14}
\@namedef{val@s2.sigma}{0.25}\@namedef{line@s2.sigma}{15}
\@namedef{val@s2.cmaseed}{424242}\@namedef{line@s2.cmaseed}{16}
\@namedef{val@s2.randseed}{535353}\@namedef{line@s2.randseed}{17}
\@namedef{val@s2.searchseeds}{3}\@namedef{line@s2.searchseeds}{18}
\@namedef{val@s2.reevalseeds}{10}\@namedef{line@s2.reevalseeds}{19}
\@namedef{val@seeds.cma}{1000--1035}\@namedef{line@seeds.cma}{20}
\@namedef{val@seeds.rand}{3000--3035}\@namedef{line@seeds.rand}{21}
\@namedef{val@seeds.fincma}{1900--1909}\@namedef{line@seeds.fincma}{22}
\@namedef{val@seeds.finrand}{3900--3909}\@namedef{line@seeds.finrand}{23}
\@namedef{val@seeds.final}{2000--2019}\@namedef{line@seeds.final}{24}
\@namedef{val@seeds.tamper}{2020--2039}\@namedef{line@seeds.tamper}{25}
\@namedef{val@s2.cap0}{\$35}\@namedef{line@s2.cap0}{26}
\@namedef{val@s3.cap0}{\$10}\@namedef{line@s3.cap0}{27}
\@namedef{val@d.h0}{0.5}\@namedef{line@d.h0}{28}
\@namedef{val@d.gmin}{1/640}\@namedef{line@d.gmin}{29}
\@namedef{val@d.gmax}{1/20}\@namedef{line@d.gmax}{30}
\@namedef{val@d.coef}{1.0}\@namedef{line@d.coef}{31}
\@namedef{val@d.resamples}{200,000}\@namedef{line@d.resamples}{32}
\@namedef{val@d.meaningful}{0.05}\@namedef{line@d.meaningful}{33}
\@namedef{val@d.delta}{0.05}\@namedef{line@d.delta}{34}
\@namedef{val@lab.gap}{0.05}\@namedef{line@lab.gap}{35}
\@namedef{val@lab.press}{1}\@namedef{line@lab.press}{36}
\@namedef{val@lab.shaping}{2}\@namedef{line@lab.shaping}{37}
\@namedef{val@lab.final}{0.9}\@namedef{line@lab.final}{38}
\@namedef{val@d.pfloor}{$5\times10^{-6}$}\@namedef{line@d.pfloor}{39}
\@namedef{val@d.ntrain}{2}\@namedef{line@d.ntrain}{40}
\@namedef{val@s1.easy}{0.85}\@namedef{line@s1.easy}{41}
\@namedef{val@s1.hard}{0.05}\@namedef{line@s1.hard}{42}
\@namedef{val@d.alpha}{0.05}\@namedef{line@d.alpha}{43}
\@namedef{val@d.window}{100}\@namedef{line@d.window}{44}
\@namedef{val@s3.runs}{340}\@namedef{line@s3.runs}{45}
\@namedef{val@s3.final}{300}\@namedef{line@s3.final}{46}
\@namedef{val@s3.tamper}{40}\@namedef{line@s3.tamper}{47}
\@namedef{val@s3.seeds}{20}\@namedef{line@s3.seeds}{48}
\@namedef{val@d.ntasks}{3}\@namedef{line@d.ntasks}{49}
\@namedef{val@d.actual}{1,998,848}\@namedef{line@d.actual}{50}
\@namedef{val@d.rows}{98}\@namedef{line@d.rows}{51}
\@namedef{val@d.finalrows}{9}\@namedef{line@d.finalrows}{52}
\@namedef{val@d.solvethr}{0.9}\@namedef{line@d.solvethr}{53}
\@namedef{val@d.holm1}{3}\@namedef{line@d.holm1}{54}
\@namedef{val@d.holm2}{6}\@namedef{line@d.holm2}{55}
\@namedef{val@d.Sgrowth}{1/160}\@namedef{line@d.Sgrowth}{56}
\@namedef{val@d.Ncoef}{$10^{-3}$}\@namedef{line@d.Ncoef}{57}
\@namedef{val@ppo.envs}{16}\@namedef{line@ppo.envs}{58}
\@namedef{val@ppo.rollout}{128}\@namedef{line@ppo.rollout}{59}
\@namedef{val@ppo.batch}{2,048}\@namedef{line@ppo.batch}{60}
\@namedef{val@ppo.gamma}{0.99}\@namedef{line@ppo.gamma}{61}
\@namedef{val@ppo.evalep}{64}\@namedef{line@ppo.evalep}{62}
\@namedef{val@reg.s1.lock}{28 October 2026, 03:12:23~UTC}\@namedef{line@reg.s1.lock}{63}
\@namedef{val@reg.s1.push}{28 October 2026, 03:12:24~UTC}\@namedef{line@reg.s1.push}{64}
\@namedef{val@reg.s2.lock}{28 October 2026, 14:28:30~UTC}\@namedef{line@reg.s2.lock}{65}
\@namedef{val@reg.s2.tested}{ae53fdd}\@namedef{line@reg.s2.tested}{66}
\@namedef{val@reg.s2.commit}{f757692}\@namedef{line@reg.s2.commit}{67}
\@namedef{val@reg.s2.push}{28 October 2026, 14:29:28~UTC}\@namedef{line@reg.s2.push}{68}
\@namedef{val@reg.s2.obs}{14:30:07~UTC}\@namedef{line@reg.s2.obs}{69}
\@namedef{val@reg.r1.commit}{490cf87}\@namedef{line@reg.r1.commit}{70}
\@namedef{val@reg.r1.public}{15:06:14~UTC}\@namedef{line@reg.r1.public}{71}
\@namedef{val@reg.r1.verified}{15:17:53~UTC}\@namedef{line@reg.r1.verified}{72}
\@namedef{val@reg.r2.commit}{cd79ce5}\@namedef{line@reg.r2.commit}{73}
\@namedef{val@reg.r2.public}{15:57:35~UTC}\@namedef{line@reg.r2.public}{74}
\@namedef{val@reg.r2.verified}{16:05:06~UTC}\@namedef{line@reg.r2.verified}{75}
\@namedef{val@reg.descsha}{46b2c8940efc}\@namedef{line@reg.descsha}{76}
\@namedef{val@reg.launch}{16:06:33~UTC}\@namedef{line@reg.launch}{77}
\@namedef{val@reg.launchdate}{29 October 2026, 16:06:33~UTC}\@namedef{line@reg.launchdate}{78}
\@namedef{val@reg.macrestart}{22:22:02~UTC}\@namedef{line@reg.macrestart}{79}
\@namedef{val@win.E}{113}\@namedef{line@win.E}{80}
\@namedef{val@win.R}{57}\@namedef{line@win.R}{81}
\@namedef{val@win.Esha}{e3ec0a9f6b76}\@namedef{line@win.Esha}{82}
\@namedef{val@win.Rsha}{f197a6444334}\@namedef{line@win.Rsha}{83}
\@namedef{val@reg.research}{7acab8c}\@namedef{line@reg.research}{84}
\@namedef{val@s3.files}{6,200}\@namedef{line@s3.files}{85}
\@namedef{val@s3.srcfiles}{62}\@namedef{line@s3.srcfiles}{86}
\@namedef{val@s3.commit}{22b0808}\@namedef{line@s3.commit}{87}
\@namedef{val@s1.DoorKey8x8.area}{0.195}\@namedef{line@s1.DoorKey8x8.area}{88}
\@namedef{val@s1.UnlockPickup.area}{0.006}\@namedef{line@s1.UnlockPickup.area}{89}
\@namedef{val@s1.KeyCorridorS3R2.area}{0.053}\@namedef{line@s1.KeyCorridorS3R2.area}{90}
\@namedef{val@s1.KeyCorridorS3R1.area}{0.855}\@namedef{line@s1.KeyCorridorS3R1.area}{91}
\@namedef{val@s1.MultiRoomN2S4.area}{0.961}\@namedef{line@s1.MultiRoomN2S4.area}{92}
\@namedef{val@s1.BlockedUnlockPickup.area}{0.008}\@namedef{line@s1.BlockedUnlockPickup.area}{93}
\@namedef{val@s1.DoorKey16x16.area}{0.045}\@namedef{line@s1.DoorKey16x16.area}{94}
\@namedef{val@s1.sep.DoorKey8x8.diff}{+0.108}\@namedef{line@s1.sep.DoorKey8x8.diff}{95}
\@namedef{val@s1.sep.DoorKey8x8.p}{0.690}\@namedef{line@s1.sep.DoorKey8x8.p}{96}
\@namedef{val@s1.sep.DoorKey8x8.ph}{1.000}\@namedef{line@s1.sep.DoorKey8x8.ph}{97}
\@namedef{val@s1.sep.KeyCorridorS3R1.diff}{+0.195}\@namedef{line@s1.sep.KeyCorridorS3R1.diff}{98}
\@namedef{val@s1.sep.KeyCorridorS3R1.p}{0.056}\@namedef{line@s1.sep.KeyCorridorS3R1.p}{99}
\@namedef{val@s1.sep.KeyCorridorS3R1.ph}{0.167}\@namedef{line@s1.sep.KeyCorridorS3R1.ph}{100}
\@namedef{val@s1.sep.UnlockPickup.diff}{+0.001}\@namedef{line@s1.sep.UnlockPickup.diff}{101}
\@namedef{val@s1.sep.UnlockPickup.p}{0.690}\@namedef{line@s1.sep.UnlockPickup.p}{102}
\@namedef{val@s1.sep.UnlockPickup.ph}{1.000}\@namedef{line@s1.sep.UnlockPickup.ph}{103}
\@namedef{val@s1.seeds}{5}\@namedef{line@s1.seeds}{104}
\@namedef{val@s1.rejected}{4}\@namedef{line@s1.rejected}{105}
\@namedef{val@s1.tooeasy}{2}\@namedef{line@s1.tooeasy}{106}
\@namedef{val@s1.toohard}{2}\@namedef{line@s1.toohard}{107}
\@namedef{val@s1.sep.count}{3}\@namedef{line@s1.sep.count}{108}
\@namedef{val@s1.det}{not bit-identical}\@namedef{line@s1.det}{109}
\@namedef{val@pin.n}{64}\@namedef{line@pin.n}{110}
\@namedef{val@pin.fp}{2}\@namedef{line@pin.fp}{111}
\@namedef{val@pin.zen3}{46}\@namedef{line@pin.zen3}{112}
\@namedef{val@pin.zen4}{5}\@namedef{line@pin.zen4}{113}
\@namedef{val@pin.intel}{13}\@namedef{line@pin.intel}{114}
\@namedef{val@s1.guard}{\$2.88}\@namedef{line@s1.guard}{115}
\@namedef{val@s1.billed}{\$1.52}\@namedef{line@s1.billed}{116}
\@namedef{val@s1.cap}{\$15}\@namedef{line@s1.cap}{117}
\@namedef{val@fin.cma92.search}{0.707}\@namedef{line@fin.cma92.search}{118}
\@namedef{val@fin.cma92.reeval}{0.587}\@namedef{line@fin.cma92.reeval}{119}
\@namedef{val@fin.cma92.change}{$-$0.120}\@namedef{line@fin.cma92.change}{120}
\@namedef{val@fin.cma113.search}{0.692}\@namedef{line@fin.cma113.search}{121}
\@namedef{val@fin.cma113.reeval}{0.596}\@namedef{line@fin.cma113.reeval}{122}
\@namedef{val@fin.cma113.change}{$-$0.096}\@namedef{line@fin.cma113.change}{123}
\@namedef{val@fin.cma94.search}{0.676}\@namedef{line@fin.cma94.search}{124}
\@namedef{val@fin.cma94.reeval}{0.497}\@namedef{line@fin.cma94.reeval}{125}
\@namedef{val@fin.cma94.change}{$-$0.179}\@namedef{line@fin.cma94.change}{126}
\@namedef{val@fin.random57.search}{0.610}\@namedef{line@fin.random57.search}{127}
\@namedef{val@fin.random57.reeval}{0.632}\@namedef{line@fin.random57.reeval}{128}
\@namedef{val@fin.random57.change}{+0.022}\@namedef{line@fin.random57.change}{129}
\@namedef{val@fin.random116.search}{0.584}\@namedef{line@fin.random116.search}{130}
\@namedef{val@fin.random116.reeval}{0.626}\@namedef{line@fin.random116.reeval}{131}
\@namedef{val@fin.random116.change}{+0.042}\@namedef{line@fin.random116.change}{132}
\@namedef{val@fin.random103.search}{0.510}\@namedef{line@fin.random103.search}{133}
\@namedef{val@fin.random103.reeval}{0.619}\@namedef{line@fin.random103.reeval}{134}
\@namedef{val@fin.random103.change}{+0.108}\@namedef{line@fin.random103.change}{135}
\@namedef{val@fin.EminusR}{$-$0.037}\@namedef{line@fin.EminusR}{136}
\@namedef{val@fin.cmafell}{3}\@namedef{line@fin.cmafell}{137}
\@namedef{val@fin.randrose}{3}\@namedef{line@fin.randrose}{138}
\@namedef{val@cand.cma.best}{0.707}\@namedef{line@cand.cma.best}{139}
\@namedef{val@cand.cma.bestid}{92}\@namedef{line@cand.cma.bestid}{140}
\@namedef{val@cand.random.best}{0.610}\@namedef{line@cand.random.best}{141}
\@namedef{val@cand.random.bestid}{57}\@namedef{line@cand.random.bestid}{142}
\@namedef{val@s2.calls}{1,802}\@namedef{line@s2.calls}{143}
\@namedef{val@s2.attempts}{1,850}\@namedef{line@s2.attempts}{144}
\@namedef{val@s2.extra}{48}\@namedef{line@s2.extra}{145}
\@namedef{val@s2.terminated}{50}\@namedef{line@s2.terminated}{146}
\@namedef{val@s2.manual}{50}\@namedef{line@s2.manual}{147}
\@namedef{val@s2.nousage}{4}\@namedef{line@s2.nousage}{148}
\@namedef{val@s2.ctrl}{5}\@namedef{line@s2.ctrl}{149}
\@namedef{val@cpu.s2.zen3}{1,266}\@namedef{line@cpu.s2.zen3}{150}
\@namedef{val@cpu.s2.intel}{205}\@namedef{line@cpu.s2.intel}{151}
\@namedef{val@cpu.s2.zen4}{61}\@namedef{line@cpu.s2.zen4}{152}
\@namedef{val@cpu.s2.other}{28}\@namedef{line@cpu.s2.other}{153}
\@namedef{val@s2.ulp}{four}\@namedef{line@s2.ulp}{154}
\@namedef{val@s2.ulpgrowth}{4}\@namedef{line@s2.ulpgrowth}{155}
\@namedef{val@cost.s2.cap}{\$50}\@namedef{line@cost.s2.cap}{156}
\@namedef{val@cost.s2.guard}{\$29.41}\@namedef{line@cost.s2.guard}{157}
\@namedef{val@cost.s2.measured}{\$22.37}\@namedef{line@cost.s2.measured}{158}
\@namedef{val@cost.s2.billed}{\$22.07}\@namedef{line@cost.s2.billed}{159}
\@namedef{val@kc.ET.diff}{+0.452}\@namedef{line@kc.ET.diff}{160}
\@namedef{val@kc.ET.gap}{0.452}\@namedef{line@kc.ET.gap}{161}
\@namedef{val@kc.ET.p}{$5\times10^{-6}$}\@namedef{line@kc.ET.p}{162}
\@namedef{val@kc.ET.ph}{$1\times10^{-5}$}\@namedef{line@kc.ET.ph}{163}
\@namedef{val@kc.ET.U}{400.0}\@namedef{line@kc.ET.U}{164}
\@namedef{val@kc.ET.hit}{hit}\@namedef{line@kc.ET.hit}{165}
\@namedef{val@kc.ET.meaningful}{yes}\@namedef{line@kc.ET.meaningful}{166}
\@namedef{val@kc.ET.method}{permutation}\@namedef{line@kc.ET.method}{167}
\@namedef{val@kc.ET.fisher}{0.053}\@namedef{line@kc.ET.fisher}{168}
\@namedef{val@kc.EN.diff}{+0.393}\@namedef{line@kc.EN.diff}{169}
\@namedef{val@kc.EN.gap}{0.393}\@namedef{line@kc.EN.gap}{170}
\@namedef{val@kc.EN.p}{$7.3\times10^{-12}$}\@namedef{line@kc.EN.p}{171}
\@namedef{val@kc.EN.ph}{$2.2\times10^{-11}$}\@namedef{line@kc.EN.ph}{172}
\@namedef{val@kc.EN.U}{400.0}\@namedef{line@kc.EN.U}{173}
\@namedef{val@kc.EN.hit}{hit}\@namedef{line@kc.EN.hit}{174}
\@namedef{val@kc.EN.meaningful}{yes}\@namedef{line@kc.EN.meaningful}{175}
\@namedef{val@kc.EN.method}{exact}\@namedef{line@kc.EN.method}{176}
\@namedef{val@kc.EN.fisher}{0.053}\@namedef{line@kc.EN.fisher}{177}
\@namedef{val@kc.ER.diff}{+0.159}\@namedef{line@kc.ER.diff}{178}
\@namedef{val@kc.ER.gap}{0.159}\@namedef{line@kc.ER.gap}{179}
\@namedef{val@kc.ER.p}{0.00015}\@namedef{line@kc.ER.p}{180}
\@namedef{val@kc.ER.ph}{0.00015}\@namedef{line@kc.ER.ph}{181}
\@namedef{val@kc.ER.U}{329.0}\@namedef{line@kc.ER.U}{182}
\@namedef{val@kc.ER.hit}{hit}\@namedef{line@kc.ER.hit}{183}
\@namedef{val@kc.ER.meaningful}{yes}\@namedef{line@kc.ER.meaningful}{184}
\@namedef{val@kc.ER.method}{exact}\@namedef{line@kc.ER.method}{185}
\@namedef{val@kc.ER.fisher}{0.053}\@namedef{line@kc.ER.fisher}{186}
\@namedef{val@kc.E.area}{0.457}\@namedef{line@kc.E.area}{187}
\@namedef{val@kc.E.sd}{0.139}\@namedef{line@kc.E.sd}{188}
\@namedef{val@kc.E.solve}{4/20}\@namedef{line@kc.E.solve}{189}
\@namedef{val@kc.E.solve.of}{4 of 20}\@namedef{line@kc.E.solve.of}{190}
\@namedef{val@kc.E.ci}{[0.06, 0.44]}\@namedef{line@kc.E.ci}{191}
\@namedef{val@kc.E.fs}{2M (censored)}\@namedef{line@kc.E.fs}{192}
\@namedef{val@kc.R.area}{0.298}\@namedef{line@kc.R.area}{193}
\@namedef{val@kc.R.sd}{0.102}\@namedef{line@kc.R.sd}{194}
\@namedef{val@kc.R.solve}{0/20}\@namedef{line@kc.R.solve}{195}
\@namedef{val@kc.R.solve.of}{0 of 20}\@namedef{line@kc.R.solve.of}{196}
\@namedef{val@kc.R.ci}{[0.00, 0.17]}\@namedef{line@kc.R.ci}{197}
\@namedef{val@kc.R.fs}{2M (censored)}\@namedef{line@kc.R.fs}{198}
\@namedef{val@kc.T.area}{0.004}\@namedef{line@kc.T.area}{199}
\@namedef{val@kc.T.sd}{0.002}\@namedef{line@kc.T.sd}{200}
\@namedef{val@kc.T.solve}{0/20}\@namedef{line@kc.T.solve}{201}
\@namedef{val@kc.T.solve.of}{0 of 20}\@namedef{line@kc.T.solve.of}{202}
\@namedef{val@kc.T.ci}{[0.00, 0.17]}\@namedef{line@kc.T.ci}{203}
\@namedef{val@kc.T.fs}{2M (censored)}\@namedef{line@kc.T.fs}{204}
\@namedef{val@kc.N.area}{0.064}\@namedef{line@kc.N.area}{205}
\@namedef{val@kc.N.sd}{0.035}\@namedef{line@kc.N.sd}{206}
\@namedef{val@kc.N.solve}{0/20}\@namedef{line@kc.N.solve}{207}
\@namedef{val@kc.N.solve.of}{0 of 20}\@namedef{line@kc.N.solve.of}{208}
\@namedef{val@kc.N.ci}{[0.00, 0.17]}\@namedef{line@kc.N.ci}{209}
\@namedef{val@kc.N.fs}{2M (censored)}\@namedef{line@kc.N.fs}{210}
\@namedef{val@kc.S.area}{0.768}\@namedef{line@kc.S.area}{211}
\@namedef{val@kc.S.sd}{0.046}\@namedef{line@kc.S.sd}{212}
\@namedef{val@kc.S.solve}{20/20}\@namedef{line@kc.S.solve}{213}
\@namedef{val@kc.S.solve.of}{20 of 20}\@namedef{line@kc.S.solve.of}{214}
\@namedef{val@kc.S.ci}{[0.83, 1.00]}\@namedef{line@kc.S.ci}{215}
\@namedef{val@kc.S.fs}{0.63M}\@namedef{line@kc.S.fs}{216}
\@namedef{val@dk.ET.diff}{+0.551}\@namedef{line@dk.ET.diff}{217}
\@namedef{val@dk.ET.gap}{0.551}\@namedef{line@dk.ET.gap}{218}
\@namedef{val@dk.ET.p}{$1.4\times10^{-9}$}\@namedef{line@dk.ET.p}{219}
\@namedef{val@dk.ET.ph}{$8.5\times10^{-9}$}\@namedef{line@dk.ET.ph}{220}
\@namedef{val@dk.ET.U}{389.0}\@namedef{line@dk.ET.U}{221}
\@namedef{val@dk.ET.hit}{hit}\@namedef{line@dk.ET.hit}{222}
\@namedef{val@dk.ET.meaningful}{yes}\@namedef{line@dk.ET.meaningful}{223}
\@namedef{val@dk.ET.method}{exact}\@namedef{line@dk.ET.method}{224}
\@namedef{val@dk.ET.fisher}{$2.3\times10^{-5}$}\@namedef{line@dk.ET.fisher}{225}
\@namedef{val@dk.EN.diff}{+0.234}\@namedef{line@dk.EN.diff}{226}
\@namedef{val@dk.EN.gap}{0.234}\@namedef{line@dk.EN.gap}{227}
\@namedef{val@dk.EN.p}{$2.1\times10^{-6}$}\@namedef{line@dk.EN.p}{228}
\@namedef{val@dk.EN.ph}{$1\times10^{-5}$}\@namedef{line@dk.EN.ph}{229}
\@namedef{val@dk.EN.U}{358.0}\@namedef{line@dk.EN.U}{230}
\@namedef{val@dk.EN.hit}{hit}\@namedef{line@dk.EN.hit}{231}
\@namedef{val@dk.EN.meaningful}{yes}\@namedef{line@dk.EN.meaningful}{232}
\@namedef{val@dk.EN.method}{exact}\@namedef{line@dk.EN.method}{233}
\@namedef{val@dk.EN.fisher}{0.115}\@namedef{line@dk.EN.fisher}{234}
\@namedef{val@dk.ER.diff}{$-$0.031}\@namedef{line@dk.ER.diff}{235}
\@namedef{val@dk.ER.gap}{$-$0.031}\@namedef{line@dk.ER.gap}{236}
\@namedef{val@dk.ER.p}{0.981}\@namedef{line@dk.ER.p}{237}
\@namedef{val@dk.ER.ph}{0.981}\@namedef{line@dk.ER.ph}{238}
\@namedef{val@dk.ER.U}{124.0}\@namedef{line@dk.ER.U}{239}
\@namedef{val@dk.ER.hit}{miss}\@namedef{line@dk.ER.hit}{240}
\@namedef{val@dk.ER.meaningful}{no}\@namedef{line@dk.ER.meaningful}{241}
\@namedef{val@dk.ER.method}{exact}\@namedef{line@dk.ER.method}{242}
\@namedef{val@dk.ER.fisher}{1.000}\@namedef{line@dk.ER.fisher}{243}
\@namedef{val@dk.E.area}{0.837}\@namedef{line@dk.E.area}{244}
\@namedef{val@dk.E.sd}{0.058}\@namedef{line@dk.E.sd}{245}
\@namedef{val@dk.E.solve}{20/20}\@namedef{line@dk.E.solve}{246}
\@namedef{val@dk.E.solve.of}{20 of 20}\@namedef{line@dk.E.solve.of}{247}
\@namedef{val@dk.E.ci}{[0.83, 1.00]}\@namedef{line@dk.E.ci}{248}
\@namedef{val@dk.E.fs}{0.45M}\@namedef{line@dk.E.fs}{249}
\@namedef{val@dk.R.area}{0.867}\@namedef{line@dk.R.area}{250}
\@namedef{val@dk.R.sd}{0.048}\@namedef{line@dk.R.sd}{251}
\@namedef{val@dk.R.solve}{20/20}\@namedef{line@dk.R.solve}{252}
\@namedef{val@dk.R.solve.of}{20 of 20}\@namedef{line@dk.R.solve.of}{253}
\@namedef{val@dk.R.ci}{[0.83, 1.00]}\@namedef{line@dk.R.ci}{254}
\@namedef{val@dk.R.fs}{0.37M}\@namedef{line@dk.R.fs}{255}
\@namedef{val@dk.T.area}{0.286}\@namedef{line@dk.T.area}{256}
\@namedef{val@dk.T.sd}{0.333}\@namedef{line@dk.T.sd}{257}
\@namedef{val@dk.T.solve}{8/20}\@namedef{line@dk.T.solve}{258}
\@namedef{val@dk.T.solve.of}{8 of 20}\@namedef{line@dk.T.solve.of}{259}
\@namedef{val@dk.T.ci}{[0.19, 0.64]}\@namedef{line@dk.T.ci}{260}
\@namedef{val@dk.T.fs}{2M (censored)}\@namedef{line@dk.T.fs}{261}
\@namedef{val@dk.N.area}{0.603}\@namedef{line@dk.N.area}{262}
\@namedef{val@dk.N.sd}{0.226}\@namedef{line@dk.N.sd}{263}
\@namedef{val@dk.N.solve}{17/20}\@namedef{line@dk.N.solve}{264}
\@namedef{val@dk.N.solve.of}{17 of 20}\@namedef{line@dk.N.solve.of}{265}
\@namedef{val@dk.N.ci}{[0.62, 0.97]}\@namedef{line@dk.N.ci}{266}
\@namedef{val@dk.N.fs}{0.86M}\@namedef{line@dk.N.fs}{267}
\@namedef{val@dk.S.area}{0.903}\@namedef{line@dk.S.area}{268}
\@namedef{val@dk.S.sd}{0.031}\@namedef{line@dk.S.sd}{269}
\@namedef{val@dk.S.solve}{20/20}\@namedef{line@dk.S.solve}{270}
\@namedef{val@dk.S.solve.of}{20 of 20}\@namedef{line@dk.S.solve.of}{271}
\@namedef{val@dk.S.ci}{[0.83, 1.00]}\@namedef{line@dk.S.ci}{272}
\@namedef{val@dk.S.fs}{0.31M}\@namedef{line@dk.S.fs}{273}
\@namedef{val@up.ET.diff}{+0.346}\@namedef{line@up.ET.diff}{274}
\@namedef{val@up.ET.gap}{0.346}\@namedef{line@up.ET.gap}{275}
\@namedef{val@up.ET.p}{$5\times10^{-6}$}\@namedef{line@up.ET.p}{276}
\@namedef{val@up.ET.ph}{$2\times10^{-5}$}\@namedef{line@up.ET.ph}{277}
\@namedef{val@up.ET.U}{399.0}\@namedef{line@up.ET.U}{278}
\@namedef{val@up.ET.hit}{hit}\@namedef{line@up.ET.hit}{279}
\@namedef{val@up.ET.meaningful}{yes}\@namedef{line@up.ET.meaningful}{280}
\@namedef{val@up.ET.method}{permutation}\@namedef{line@up.ET.method}{281}
\@namedef{val@up.ET.fisher}{0.002}\@namedef{line@up.ET.fisher}{282}
\@namedef{val@up.EN.diff}{+0.342}\@namedef{line@up.EN.diff}{283}
\@namedef{val@up.EN.gap}{0.342}\@namedef{line@up.EN.gap}{284}
\@namedef{val@up.EN.p}{$5\times10^{-6}$}\@namedef{line@up.EN.p}{285}
\@namedef{val@up.EN.ph}{$2\times10^{-5}$}\@namedef{line@up.EN.ph}{286}
\@namedef{val@up.EN.U}{396.0}\@namedef{line@up.EN.U}{287}
\@namedef{val@up.EN.hit}{hit}\@namedef{line@up.EN.hit}{288}
\@namedef{val@up.EN.meaningful}{yes}\@namedef{line@up.EN.meaningful}{289}
\@namedef{val@up.EN.method}{permutation}\@namedef{line@up.EN.method}{290}
\@namedef{val@up.EN.fisher}{0.002}\@namedef{line@up.EN.fisher}{291}
\@namedef{val@up.ER.diff}{+0.055}\@namedef{line@up.ER.diff}{292}
\@namedef{val@up.ER.gap}{0.055}\@namedef{line@up.ER.gap}{293}
\@namedef{val@up.ER.p}{0.192}\@namedef{line@up.ER.p}{294}
\@namedef{val@up.ER.ph}{0.383}\@namedef{line@up.ER.ph}{295}
\@namedef{val@up.ER.U}{233.0}\@namedef{line@up.ER.U}{296}
\@namedef{val@up.ER.hit}{miss}\@namedef{line@up.ER.hit}{297}
\@namedef{val@up.ER.meaningful}{no}\@namedef{line@up.ER.meaningful}{298}
\@namedef{val@up.ER.method}{exact}\@namedef{line@up.ER.method}{299}
\@namedef{val@up.ER.fisher}{0.078}\@namedef{line@up.ER.fisher}{300}
\@namedef{val@up.E.area}{0.349}\@namedef{line@up.E.area}{301}
\@namedef{val@up.E.sd}{0.187}\@namedef{line@up.E.sd}{302}
\@namedef{val@up.E.solve}{8/20}\@namedef{line@up.E.solve}{303}
\@namedef{val@up.E.solve.of}{8 of 20}\@namedef{line@up.E.solve.of}{304}
\@namedef{val@up.E.ci}{[0.19, 0.64]}\@namedef{line@up.E.ci}{305}
\@namedef{val@up.E.fs}{1.68M}\@namedef{line@up.E.fs}{306}
\@namedef{val@up.R.area}{0.294}\@namedef{line@up.R.area}{307}
\@namedef{val@up.R.sd}{0.134}\@namedef{line@up.R.sd}{308}
\@namedef{val@up.R.solve}{3/20}\@namedef{line@up.R.solve}{309}
\@namedef{val@up.R.solve.of}{3 of 20}\@namedef{line@up.R.solve.of}{310}
\@namedef{val@up.R.ci}{[0.03, 0.38]}\@namedef{line@up.R.ci}{311}
\@namedef{val@up.R.fs}{2M (censored)}\@namedef{line@up.R.fs}{312}
\@namedef{val@up.T.area}{0.003}\@namedef{line@up.T.area}{313}
\@namedef{val@up.T.sd}{0.002}\@namedef{line@up.T.sd}{314}
\@namedef{val@up.T.solve}{0/20}\@namedef{line@up.T.solve}{315}
\@namedef{val@up.T.solve.of}{0 of 20}\@namedef{line@up.T.solve.of}{316}
\@namedef{val@up.T.ci}{[0.00, 0.17]}\@namedef{line@up.T.ci}{317}
\@namedef{val@up.T.fs}{2M (censored)}\@namedef{line@up.T.fs}{318}
\@namedef{val@up.N.area}{0.006}\@namedef{line@up.N.area}{319}
\@namedef{val@up.N.sd}{0.002}\@namedef{line@up.N.sd}{320}
\@namedef{val@up.N.solve}{0/20}\@namedef{line@up.N.solve}{321}
\@namedef{val@up.N.solve.of}{0 of 20}\@namedef{line@up.N.solve.of}{322}
\@namedef{val@up.N.ci}{[0.00, 0.17]}\@namedef{line@up.N.ci}{323}
\@namedef{val@up.N.fs}{2M (censored)}\@namedef{line@up.N.fs}{324}
\@namedef{val@up.S.area}{0.073}\@namedef{line@up.S.area}{325}
\@namedef{val@up.S.sd}{0.143}\@namedef{line@up.S.sd}{326}
\@namedef{val@up.S.solve}{1/20}\@namedef{line@up.S.solve}{327}
\@namedef{val@up.S.solve.of}{1 of 20}\@namedef{line@up.S.solve.of}{328}
\@namedef{val@up.S.ci}{[0.00, 0.25]}\@namedef{line@up.S.ci}{329}
\@namedef{val@up.S.fs}{2M (censored)}\@namedef{line@up.S.fs}{330}
\@namedef{val@kc.hits}{3}\@namedef{line@kc.hits}{331}
\@namedef{val@kc.meaningful}{3}\@namedef{line@kc.meaningful}{332}
\@namedef{val@sec.hits}{4}\@namedef{line@sec.hits}{333}
\@namedef{val@kc.SminusE}{+0.311}\@namedef{line@kc.SminusE}{334}
\@namedef{val@up.EminusS}{+0.276}\@namedef{line@up.EminusS}{335}
\@namedef{val@up.EminusS.gap}{0.276}\@namedef{line@up.EminusS.gap}{336}
\@namedef{val@tam.P0}{0.6396}\@namedef{line@tam.P0}{337}
\@namedef{val@tam.P0full}{0.6396352350711823}\@namedef{line@tam.P0full}{338}
\@namedef{val@tam.P0five}{0.63964}\@namedef{line@tam.P0five}{339}
\@namedef{val@tam.off.area}{0.829}\@namedef{line@tam.off.area}{340}
\@namedef{val@tam.on.area}{0.136}\@namedef{line@tam.on.area}{341}
\@namedef{val@tam.diff}{0.693}\@namedef{line@tam.diff}{342}
\@namedef{val@tam.p}{$5\times10^{-6}$}\@namedef{line@tam.p}{343}
\@namedef{val@tam.U}{393.0}\@namedef{line@tam.U}{344}
\@namedef{val@tam.solve.off}{20/20}\@namedef{line@tam.solve.off}{345}
\@namedef{val@tam.solve.on}{4/20}\@namedef{line@tam.solve.on}{346}
\@namedef{val@tam.vsT}{$-$0.150}\@namedef{line@tam.vsT}{347}
\@namedef{val@tam.vsT.gap}{0.150}\@namedef{line@tam.vsT.gap}{348}
\@namedef{val@tam.label}{wireheading-like}\@namedef{line@tam.label}{349}
\@namedef{val@tam.medmin}{45.9}\@namedef{line@tam.medmin}{350}
\@namedef{val@tam.medmax}{48.0}\@namedef{line@tam.medmax}{351}
\@namedef{val@tam.windows}{11}\@namedef{line@tam.windows}{352}
\@namedef{val@tam.on.pps10}{7.9\%}\@namedef{line@tam.on.pps10}{353}
\@namedef{val@tam.on.pps10b}{7.864\%}\@namedef{line@tam.on.pps10b}{354}
\@namedef{val@tam.on.pps}{10.3\%}\@namedef{line@tam.on.pps}{355}
\@namedef{val@tam.on.ppe10}{39.4}\@namedef{line@tam.on.ppe10}{356}
\@namedef{val@tam.on.ppe}{52.4}\@namedef{line@tam.on.ppe}{357}
\@namedef{val@tam.on.iret}{0.637}\@namedef{line@tam.on.iret}{358}
\@namedef{val@tam.on.iret10}{0.636}\@namedef{line@tam.on.iret10}{359}
\@namedef{val@tam.on.iretmax}{0.63964}\@namedef{line@tam.on.iretmax}{360}
\@namedef{val@tam.on.aboveP0}{0}\@namedef{line@tam.on.aboveP0}{361}
\@namedef{val@tam.on.above064}{0}\@namedef{line@tam.on.above064}{362}
\@namedef{val@tam.on.ent}{1.634}\@namedef{line@tam.on.ent}{363}
\@namedef{val@tam.on.ent9}{1.516}\@namedef{line@tam.on.ent9}{364}
\@namedef{val@tam.off.pps10}{0.0\%}\@namedef{line@tam.off.pps10}{365}
\@namedef{val@tam.off.pps10b}{0.004\%}\@namedef{line@tam.off.pps10b}{366}
\@namedef{val@tam.off.pps}{1.4\%}\@namedef{line@tam.off.pps}{367}
\@namedef{val@tam.off.ppe10}{0.0}\@namedef{line@tam.off.ppe10}{368}
\@namedef{val@tam.off.ppe}{0.6}\@namedef{line@tam.off.ppe}{369}
\@namedef{val@tam.off.iret}{0.592}\@namedef{line@tam.off.iret}{370}
\@namedef{val@tam.off.iret10}{0.607}\@namedef{line@tam.off.iret10}{371}
\@namedef{val@tam.off.iretmax}{0.63964}\@namedef{line@tam.off.iretmax}{372}
\@namedef{val@tam.off.aboveP0}{1}\@namedef{line@tam.off.aboveP0}{373}
\@namedef{val@tam.off.above064}{0}\@namedef{line@tam.off.above064}{374}
\@namedef{val@tam.off.ent}{0.787}\@namedef{line@tam.off.ent}{375}
\@namedef{val@tam.off.ent9}{0.387}\@namedef{line@tam.off.ent9}{376}
\@namedef{val@tam.off.excess}{$2.9\times10^{-9}$}\@namedef{line@tam.off.excess}{377}
\@namedef{val@tam.uniform}{14.3\%}\@namedef{line@tam.uniform}{378}
\@namedef{val@tam.ln7}{1.946}\@namedef{line@tam.ln7}{379}
\@namedef{val@g.E.newview.w}{0.554}\@namedef{line@g.E.newview.w}{380}
\@namedef{val@g.E.newview.s}{0.928}\@namedef{line@g.E.newview.s}{381}
\@namedef{val@g.E.newview.g}{0.0039}\@namedef{line@g.E.newview.g}{382}
\@namedef{val@g.E.newview.period}{258}\@namedef{line@g.E.newview.period}{383}
\@namedef{val@g.E.newview.once}{no}\@namedef{line@g.E.newview.once}{384}
\@namedef{val@g.E.pickup.w}{0.632}\@namedef{line@g.E.pickup.w}{385}
\@namedef{val@g.E.pickup.s}{0.633}\@namedef{line@g.E.pickup.s}{386}
\@namedef{val@g.E.pickup.g}{0}\@namedef{line@g.E.pickup.g}{387}
\@namedef{val@g.E.pickup.period}{--}\@namedef{line@g.E.pickup.period}{388}
\@namedef{val@g.E.pickup.once}{yes}\@namedef{line@g.E.pickup.once}{389}
\@namedef{val@g.E.drop.w}{0.966}\@namedef{line@g.E.drop.w}{390}
\@namedef{val@g.E.drop.s}{0.564}\@namedef{line@g.E.drop.s}{391}
\@namedef{val@g.E.drop.g}{0}\@namedef{line@g.E.drop.g}{392}
\@namedef{val@g.E.drop.period}{--}\@namedef{line@g.E.drop.period}{393}
\@namedef{val@g.E.drop.once}{yes}\@namedef{line@g.E.drop.once}{394}
\@namedef{val@g.E.toggle.w}{0.406}\@namedef{line@g.E.toggle.w}{395}
\@namedef{val@g.E.toggle.s}{0.690}\@namedef{line@g.E.toggle.s}{396}
\@namedef{val@g.E.toggle.g}{0}\@namedef{line@g.E.toggle.g}{397}
\@namedef{val@g.E.toggle.period}{--}\@namedef{line@g.E.toggle.period}{398}
\@namedef{val@g.E.toggle.once}{yes}\@namedef{line@g.E.toggle.once}{399}
\@namedef{val@g.R.newview.w}{0.368}\@namedef{line@g.R.newview.w}{400}
\@namedef{val@g.R.newview.s}{0.803}\@namedef{line@g.R.newview.s}{401}
\@namedef{val@g.R.newview.g}{0.0086}\@namedef{line@g.R.newview.g}{402}
\@namedef{val@g.R.newview.period}{117}\@namedef{line@g.R.newview.period}{403}
\@namedef{val@g.R.newview.once}{no}\@namedef{line@g.R.newview.once}{404}
\@namedef{val@g.R.pickup.w}{0.039}\@namedef{line@g.R.pickup.w}{405}
\@namedef{val@g.R.pickup.s}{0.483}\@namedef{line@g.R.pickup.s}{406}
\@namedef{val@g.R.pickup.g}{0}\@namedef{line@g.R.pickup.g}{407}
\@namedef{val@g.R.pickup.period}{--}\@namedef{line@g.R.pickup.period}{408}
\@namedef{val@g.R.pickup.once}{no}\@namedef{line@g.R.pickup.once}{409}
\@namedef{val@g.R.drop.w}{$-$0.106}\@namedef{line@g.R.drop.w}{410}
\@namedef{val@g.R.drop.s}{0.014}\@namedef{line@g.R.drop.s}{411}
\@namedef{val@g.R.drop.g}{0.0027}\@namedef{line@g.R.drop.g}{412}
\@namedef{val@g.R.drop.period}{367}\@namedef{line@g.R.drop.period}{413}
\@namedef{val@g.R.drop.once}{no}\@namedef{line@g.R.drop.once}{414}
\@namedef{val@g.R.toggle.w}{0.399}\@namedef{line@g.R.toggle.w}{415}
\@namedef{val@g.R.toggle.s}{0.966}\@namedef{line@g.R.toggle.s}{416}
\@namedef{val@g.R.toggle.g}{0}\@namedef{line@g.R.toggle.g}{417}
\@namedef{val@g.R.toggle.period}{--}\@namedef{line@g.R.toggle.period}{418}
\@namedef{val@g.R.toggle.once}{yes}\@namedef{line@g.R.toggle.once}{419}
\@namedef{val@g.R.droppenalty}{0.003}\@namedef{line@g.R.droppenalty}{420}
\@namedef{val@cpu.s3.zen3}{264}\@namedef{line@cpu.s3.zen3}{421}
\@namedef{val@cpu.s3.intel}{61}\@namedef{line@cpu.s3.intel}{422}
\@namedef{val@cpu.s3.zen4}{20}\@namedef{line@cpu.s3.zen4}{423}
\@namedef{val@cpu.s3.other}{8}\@namedef{line@cpu.s3.other}{424}
\@namedef{val@s3.extra}{13}\@namedef{line@s3.extra}{425}
\@namedef{val@s3.manual}{0}\@namedef{line@s3.manual}{426}
\@namedef{val@s3.ctrl}{0}\@namedef{line@s3.ctrl}{427}
\@namedef{val@s3.handles}{374}\@namedef{line@s3.handles}{428}
\@namedef{val@cost.s3.cap}{\$15}\@namedef{line@cost.s3.cap}{429}
\@namedef{val@cost.s3.guard}{\$7.04}\@namedef{line@cost.s3.guard}{430}
\@namedef{val@cost.s3.measured}{\$4.81}\@namedef{line@cost.s3.measured}{431}
\@namedef{val@cost.s3.billed}{\$5.08}\@namedef{line@cost.s3.billed}{432}
\@namedef{val@s3.lid}{waived, unverified}\@namedef{line@s3.lid}{433}
\@namedef{val@x.pooled.toggle.positive}{0.351}\@namedef{line@x.pooled.toggle.positive}{434}
\@namedef{val@x.pooled.toggle.positive.n}{160}\@namedef{line@x.pooled.toggle.positive.n}{435}
\@namedef{val@x.random.toggle.positive}{0.204}\@namedef{line@x.random.toggle.positive}{436}
\@namedef{val@x.random.toggle.positive.n}{61}\@namedef{line@x.random.toggle.positive.n}{437}
\@namedef{val@x.pooled.toggle.negative}{0.075}\@namedef{line@x.pooled.toggle.negative}{438}
\@namedef{val@x.pooled.toggle.negative.n}{80}\@namedef{line@x.pooled.toggle.negative.n}{439}
\@namedef{val@x.random.toggle.negative}{0.068}\@namedef{line@x.random.toggle.negative}{440}
\@namedef{val@x.random.toggle.negative.n}{59}\@namedef{line@x.random.toggle.negative.n}{441}
\@namedef{val@x.pooled.toggle.zero}{0.307}\@namedef{line@x.pooled.toggle.zero}{442}
\@namedef{val@x.pooled.toggle.zero.n}{156}\@namedef{line@x.pooled.toggle.zero.n}{443}
\@namedef{val@x.random.toggle.zero}{0.160}\@namedef{line@x.random.toggle.zero}{444}
\@namedef{val@x.random.toggle.zero.n}{66}\@namedef{line@x.random.toggle.zero.n}{445}
\@namedef{val@x.pooled.toggle.nonzero}{0.170}\@namedef{line@x.pooled.toggle.nonzero}{446}
\@namedef{val@x.pooled.toggle.nonzero.n}{84}\@namedef{line@x.pooled.toggle.nonzero.n}{447}
\@namedef{val@x.random.toggle.nonzero}{0.110}\@namedef{line@x.random.toggle.nonzero}{448}
\@namedef{val@x.random.toggle.nonzero.n}{54}\@namedef{line@x.random.toggle.nonzero.n}{449}
\@namedef{val@x.rho.pooled.toggle}{0.53}\@namedef{line@x.rho.pooled.toggle}{450}
\@namedef{val@x.rho.random.toggle}{0.21}\@namedef{line@x.rho.random.toggle}{451}
\@namedef{val@x.pooled.pickup.positive}{0.320}\@namedef{line@x.pooled.pickup.positive}{452}
\@namedef{val@x.pooled.pickup.positive.n}{172}\@namedef{line@x.pooled.pickup.positive.n}{453}
\@namedef{val@x.random.pickup.positive}{0.183}\@namedef{line@x.random.pickup.positive}{454}
\@namedef{val@x.random.pickup.positive.n}{71}\@namedef{line@x.random.pickup.positive.n}{455}
\@namedef{val@x.pooled.pickup.negative}{0.106}\@namedef{line@x.pooled.pickup.negative}{456}
\@namedef{val@x.pooled.pickup.negative.n}{68}\@namedef{line@x.pooled.pickup.negative.n}{457}
\@namedef{val@x.random.pickup.negative}{0.071}\@namedef{line@x.random.pickup.negative}{458}
\@namedef{val@x.random.pickup.negative.n}{49}\@namedef{line@x.random.pickup.negative.n}{459}
\@namedef{val@x.pooled.pickup.zero}{0.338}\@namedef{line@x.pooled.pickup.zero}{460}
\@namedef{val@x.pooled.pickup.zero.n}{136}\@namedef{line@x.pooled.pickup.zero.n}{461}
\@namedef{val@x.random.pickup.zero}{0.176}\@namedef{line@x.random.pickup.zero}{462}
\@namedef{val@x.random.pickup.zero.n}{53}\@namedef{line@x.random.pickup.zero.n}{463}
\@namedef{val@x.pooled.pickup.nonzero}{0.156}\@namedef{line@x.pooled.pickup.nonzero}{464}
\@namedef{val@x.pooled.pickup.nonzero.n}{104}\@namedef{line@x.pooled.pickup.nonzero.n}{465}
\@namedef{val@x.random.pickup.nonzero}{0.107}\@namedef{line@x.random.pickup.nonzero}{466}
\@namedef{val@x.random.pickup.nonzero.n}{67}\@namedef{line@x.random.pickup.nonzero.n}{467}
\@namedef{val@x.rho.pooled.pickup}{0.37}\@namedef{line@x.rho.pooled.pickup}{468}
\@namedef{val@x.rho.random.pickup}{0.33}\@namedef{line@x.rho.random.pickup}{469}
\@namedef{val@x.pooled.drop.positive}{0.296}\@namedef{line@x.pooled.drop.positive}{470}
\@namedef{val@x.pooled.drop.positive.n}{147}\@namedef{line@x.pooled.drop.positive.n}{471}
\@namedef{val@x.random.drop.positive}{0.105}\@namedef{line@x.random.drop.positive}{472}
\@namedef{val@x.random.drop.positive.n}{61}\@namedef{line@x.random.drop.positive.n}{473}
\@namedef{val@x.pooled.drop.negative}{0.201}\@namedef{line@x.pooled.drop.negative}{474}
\@namedef{val@x.pooled.drop.negative.n}{93}\@namedef{line@x.pooled.drop.negative.n}{475}
\@namedef{val@x.random.drop.negative}{0.171}\@namedef{line@x.random.drop.negative}{476}
\@namedef{val@x.random.drop.negative.n}{59}\@namedef{line@x.random.drop.negative.n}{477}
\@namedef{val@x.pooled.drop.zero}{0.299}\@namedef{line@x.pooled.drop.zero}{478}
\@namedef{val@x.pooled.drop.zero.n}{146}\@namedef{line@x.pooled.drop.zero.n}{479}
\@namedef{val@x.random.drop.zero}{0.133}\@namedef{line@x.random.drop.zero}{480}
\@namedef{val@x.random.drop.zero.n}{59}\@namedef{line@x.random.drop.zero.n}{481}
\@namedef{val@x.pooled.drop.nonzero}{0.197}\@namedef{line@x.pooled.drop.nonzero}{482}
\@namedef{val@x.pooled.drop.nonzero.n}{94}\@namedef{line@x.pooled.drop.nonzero.n}{483}
\@namedef{val@x.random.drop.nonzero}{0.142}\@namedef{line@x.random.drop.nonzero}{484}
\@namedef{val@x.random.drop.nonzero.n}{61}\@namedef{line@x.random.drop.nonzero.n}{485}
\@namedef{val@x.rho.pooled.drop}{0.27}\@namedef{line@x.rho.pooled.drop}{486}
\@namedef{val@x.rho.random.drop}{$-$0.13}\@namedef{line@x.rho.random.drop}{487}
\@namedef{val@x.sixteen}{1/16}\@namedef{line@x.sixteen}{488}
\@namedef{val@x.sixteenpct}{6.25\%}\@namedef{line@x.sixteenpct}{489}
\makeatother

